Learning Multi-Granular Spatio-Temporal Graph Network for Skeleton-based Action Recognition

The task of skeleton-based action recognition remains a core challenge in human-centred scene understanding due to the multiple granularities and large variation in human motion. Existing approaches typically employ a single neural representation for different motion patterns, which has difficulty in capturing fine-grained action classes given limited training data. To address the aforementioned problems, we propose a novel multi-granular spatio-temporal graph network for skeleton-based action classification that jointly models the coarse- and fine-grained skeleton motion patterns. To this end, we develop a dual-head graph network consisting of two interleaved branches, which enables us to extract features at two spatio-temporal resolutions in an effective and efficient manner. Moreover, our network utilises a cross-head communication strategy to mutually enhance the representations of both heads. We conducted extensive experiments on three large-scale datasets, namely NTU RGB+D 60, NTU RGB+D 120, and Kinetics-Skeleton, and achieves the state-of-the-art performance on all the benchmarks, which validates the effectiveness of our method.

==> paperSec/abstract.tex <==
\begin{abstract}
    In our paper, we propose a dual-head graph convolution network for skeleton-based action recognition, in order to jointly capture fine grained and coarse grained motion patterns efficiently. Existing GCN based methods encode different granularities of motion patterns in a unified representation. In dual head network, each head focuses on specific granularity of temporal motions and hence is more effective. We further propose a cross head attention strategy to communicate the information of each other. 
    We conduct extensive experiments on three large-scale datasets, namely NTU RGB+D 60, NTU RGB+D120, and Kinetics-Skeleton. Our model achieves State-of-the-Art performance on all of the above benchmarks.
    
%    In our model, one branch focuses on extracting joint-level semantic features, and the other branch focuses on extracting detailed temporal motion information. In the end, we are able to fuse the outputs of both networks, performing joint spatial and temporal inference. 
    
    
  %  In this paper, we propose a coarse-fine dual head graph convolution network for skeleton based action recognition, in order to jointly capture fine grained and coarse grained motion patterns efficiently. Our fine head is able to capture fine grained motion contexts while our coarse head focuses on coarse grained motion contexts. We also propose a cross head temporal attention to pass fine grained context from fine head to coarse head, and a spatial attention to pass coarse grained contexts from coarse head to fine head. The proposed attention mechanism is able to guide the two head communicating sufficiently. Moreover, each head generates a prediction of action probabilities, and we fuse the information of two heads in a score level fusion. In addition, we perform simplification to GCN blocks in both fine head and coarse head to reduce model complexity. As a result, our proposed network is able to achieve new state-of-the-art on three public benchmarks, namely NTURGBD-60, NTURGBD-120 and kinetics dataset with fewer parameters compared to our baseline method MS-G3D, demonstrating the effectiveness of our proposed coarse-fine dual head network.
    
    
\end{abstract}

==> paperSec/intro-jiange.tex <==

\section{Introduction}

Action recognition is a fundamental problem in computer vision. Recently, skeleton-based action recognition has attracted increasing attention to the community due to the advent of cheap motion sensors \cite{cao2018openpose,ntu_60} and effective human pose estimation algorithms\cite{st-gcn,2s-agcn,ms-g3d}. Accurately recognizing actions from skeleton data can be very helpful in human-computer interactions, healthcare assistance or physical education. 

%\vspace{5cm}
Different from RGB videos, skeleton data only contains the 2D or 3D coordinates of the human joints and lack of image level contextual information. This causes the task of skeleton-based action recognition very challenging. The key to recognizing skeleton-based action is to explore discriminative spatial structure and temporal motion patterns. Due to the lack of image level contexts, existing methods\cite{ms-aagcn,st-gcn,ms-g3d} usually sample the skeleton data at the original frame rate of skeleton sequence. In this way, the input data of the network carry sufficient fine-grained temporal motion information, and hence is able to predict reasonable action probabilities from skeleton data despite the lack of image contexts. But it is still limited in learning multi-granularities and fine-grained representation of actions.

On the one hand, the motion of different joints within an action always appear to be distinct at temporal granurity. For example, 'clapping' refreshes relatively slowly in visual appearance of human body, while performs fast motion at hands. \cite{slowfast} proposed a slow-fast modeling approach which performs promisingly in RGB-based action recognition task. Unfortunately, to the best of our knowledge, such different granurities of temporal motion information are not sufficient explored in recent GCN based networks. Prior GCN based methods\cite{ms-aagcn,st-gcn,ms-g3d} couple different granularities of temporal motions in a unified representation, which is ineffective. We argue that recognizing actions represented by skeleton sequences also needs to model motion patterns of different temporal granularities.

On the other hand, some actions may only differ remarkably in a small section of time span and the motion of a portion of human joints. For example, To distinguish 'put on a shoe' and 'take off a shoe', one need to pay attention at the joints of hands and foots and the time span during which the interaction of these joints occurs. However, existing methods still work not very well in recognizing actions with fine-grained difference. Multi-granurities can alleviate these problem to a certain extent, because the fast branch and the slow branch can lay emphasis on temporal domain and spatial domain respectively due to their different manners of feature construction\cite{slowfast}. But they still have drawbacks, as the fast branch is poor in the ability of "where to look" and slow branch is poor in "when to attend".
 
In this paper, we propose a dual head framework in order to capture both coarse grained and fine grained motion contexts effectively. Our key idea is to utilize two branch of networks to extract features at two different temporal resolutions. The branch with lower temporal resolution captures motion patterns in a coarse level, while the branch with higher temporal resolution is able to encode more subtle temporal movements. Such coarse level feature extraction and fine level feature extraction are parallelly processed and finally the outputs of both branches are fused to perform dual-granularity reasoning.

To achieve this, we first take all frames of skeleton sequence and feed it into a backbone GCN. The backbone network extracts low level spatial and temporal features. Then we perform two different operations to the resulting feature maps: in one operation we subsample the feature maps at temporal dimension with a downsampling rate, such operation removes the detailed motion information and hence produces a coarse grained representation; in the other operation we utilize an identity mapping to get a fine grained representation. Then we utilize two types of GCN blocks to process the resulting coarse grained and fine grained representations. 

\begin{figure}[!tbp]
	\includegraphics[width=0.5\textwidth]{paperSec/imgs/ad_picture/ads.pdf}
	\caption{Some actions can be recognized via coarse grained temporal motion patterns(first sample), while recognizing other actions requires not only coarse grained motion but subtle temporal movements(second sample).}
	\label{fig:advertisment}
\end{figure}

Specifically, the two representations with different granularities are processed in two branches, which are referred as \textit{fine head} and \textit{coarse head}. Each head consists of two GCN blocks, which iteratively extract features with respective granularity. Our coarse head captures the correlations between joints at lower temporal resolution, hence infers actions in a more holistic way. To facilitate such coarse level inference, we utilize the fine grained feature representation in fine head to estimate a temporal attention, which indicates the importance of each frame. The temporal attention is utilized to re-weight the features at coarse head. Similarly, we utilize the coarse grained features to estimate a spatial attention indicating the joint level importance. The spatial attention is utilized to highlight the pivotal joint nodes in fine head. Our fine GCN blocks are able to focus on the subtle temporal movements of the pivotal joints and hence extract the fine-grained information effectively. 

Moreover, our dual granularity head consists of two stages. At each stage, a fine GCN block extracts fine grained features at higher temporal resolution, and then generates a temporal attention based on its resulting feature map. Then our coarse head re-weights the coarse level feature with the temporal attention, and further utilizes a coarse GCN block to perform coarse level inference. At last, we predict a joint level spatial attention based on the coarse representation, which is used to enhance fine grained features by re-weighting. Such processes are alternately processed in each stage. Finally, each head predicts an action score, and the final prediction is given by fusion of two scores.

We conduct the experiments on three public datasets: NTU-60, NTU-120, Kinetics-Skeleton. As a result, our method outperforms existing works in all benchmarks, achieving new state-of-the-art, demonstrating the effectiveness of the proposed coarse-and-fine dual head structure. To summarize our contributions, we:

% 1). propose a dual head network that two heads are slightly different in temporal resolution or channel 
% dimensions, aiming to joint capture spatial and temporal context effectively;

% 2). propose a cross branch attention mechanism to enhance the spatial and temporal features of both heads, the attentions are used for fusing information of two heads. \textcolor{blue}{Alternating strategy}

% 2). propose a voting mechanism to skeleton-based action recognition, which simply fuses the predictions of both heads. 

% 4). achieve new state-of-the-art on three public benchmarks.

1). propose a dual head architecture which can effectively learn robust representations from temporal coarse-level and fine-level for skeleton sequence data.

2). propose a cross head attention mechanism to mutually enhance the features of both heads in an alternative manner. 

3). achieve new state-of-the-art on three public benchmarks.




% Specifically, each stage consists of three steps. At step one, a fine GCN block first processes the fine grained representation, and then estimates a temporal attention based on resulting fine features. The temporal attention indicates the importance of each frame, which is used to re-weight the features in coarse head. At step two, a coarse GCN block updates coarse feature and estimate a spatial attention based on the resulting coarse representation, which indicates the importance of each joint. At step three, the fine grained feature is re-weighted by the spatial attention from coarse head. The intuition 



% \vspace{5cm}

%Our key idea is to sub-sample the frames at temporal dimension to maintain an additional coarse branch. Since we have reduced the frame rate, the adjacent feature frames are actually long range in their original temporal resolution. Due to sub-sampling process, we have removed the fine-grained temporal motion contexts and hence the network will focus on long range modeling. 

% To achieve this, we propose a coarse-fine dual head network. Our network consists of three modules: a backbone module extracts low level spatial and temporal features; a coarse-fine dual head module to encode both short-term and long-term dependencies; and a voting module to aggregates the short-term information and long-term information via score level fusion. We adopt the basic GCN block in previous work \cite{ms-g3d} as our backbone module. Our coarse-fine dual head module consists of a fine head and a coarse to model short-term and long-term dependencies. Specifically, in our fine head, multiple GCN blocks are concatenated to extract fine-grained motion contexts from the features with high temporal resolution. Meanwhile, in the coarse head, another bunch of GCN blocks are concatenated to extract long range motion dependencies at the down-sampled temporal resolution. To further improve the cross head context fusion and facilitate long range dependency modeling, we propose a cross head temporal attention block, which takes the feature maps from fine head to estimate a temporal attention, indicating the importance of each frame. The temporal attention is then utilized to re-weight the features in the coarse head. Moreover, we propose a cross head spatial attention mechanism, which takes the feature maps from coarse head to estimate a spatial attention, indicating the importance of each joint. The spatial attention is shared in all frames, and passes long range contexts from coarse head to fine head, to enhance fine representations. Such cross head temporal attention and spatial attention is alternately performed though forward process of dual heads, achieving efficient short-term and long-term dependency modeling. In the last stage, our voting module first predicts the action scores via each head, and then fuses the predictions via weighted sum. 





%Understanding actions from a skeleton sequence reuqires different granularities of motion patterns, existing works encodes multiple grained motion information in a unified representation, which is inefficient. Our method captures coarse grained and fine grained motion patterns in two different heads, hence is more robust to fine-grained action classes, e.g. 'reading' and 'writing'.



%\vspace{5cm}




%  Action recognition is a fundamental problem in computer vision. Recently, skeleton-based action recognition have attracted increasing attention due to the light-weight data source, high-level semantic information and robustness against complicated environment\cite{st-gcn,2s-agcn,ms-g3d}.  (Wang et al. 2018; Vemulapalli, Arrate, andChellappa 2014; Liu, Liu, and Chen 2017; Tu, Liu, and Liu2018). 
 
%  The advent of cheap motion sensors \cite{kinect,ntu_60} and effective human pose estimation algorithms  \cite{st-gcn,2s-agcn,ms-g3d} further speed up this research topic. 
%  Accurately recognizing actions from skeletal data can be very helpful in human-computer interactions, healthcare assistance and physical education\cite{xxx}. 

% related work
% Different from RGB videos, skeleton data only contains the 2D or 3D coordinates of the human key joints and lacks of image level contextual information. Hence our designed model should focus on the structure of human and motion patterns of skeletal joints. This causes the task of skeleton-based action recognition very challenging. 
% Existing works mainly focus on extracting discriminative spatial and temporal features of skeletal joints \cite{ms-aagcn,st-gcn}. Recent deep network based methods can be categorized into three types: RNNs, CNNs and GCNs. First of all, a typical method of skeleton based action recognition is RNNs\cite{xx}. Those methods first extract frame level skeletal features with a feature extractor and then modeling sequential dependencies with RNN models\cite{xx}. Typical drawback of those methods is that they compress the joint data to person-level feature in each frame and hence the intra-joint dependencies in temporal domain are hard to capture \cite{st-gcn}. The second pipeline for skeleton-based action recognition can be summarized as CNNs\cite{xxx}, which treat the joint positional data as pixels. They first flatten skeletal data of each frame to a column of pixels and then stack multiple frame data to generate an pesudo-image. Finally image-based classification CNNs are used for action recognition. However, as human skeletons lie in a non-Euclidean space, directly stacking different joints together and utilizing convolution operations may not be effective in modeling joint-level dependencies. The third framework of our task is GCNs\cite{st-gcn}, which are widely adopted in recent years due to their efficacy in spatial and temporal modeling. A milestone of GCN-based method is ST-GCN\cite{st-gcn}, which defines a sparse connected spatial-temporal graph that both considers human natural structure and temporal motion dependencies in space-time domain. Since then, many works attempted to improve the graph topology by making the graph connections learnable\cite{2s-agcn, dynamic_gcn}, adding residual layers\cite{ResGCN},  exploring contextual information between joints\cite{zhang2020context}, or introducing multi-scale spatial connections\cite{ms-g3d}.  


%allowing action recognition models to focus on understanding the action itself.
% For example, we can not infer which sport of a sport player is playing by his clothes or environments but only the skeletal sequence. This causes the task of skeleton-based action recognition very challenging. 

% In recent years, deep learning based methods have been the dominant stream for skeleton-based action recognition\cite{st-gcn, ms-aagcn,ms-g3d,decouple_gcn_cheng2020eccv,shift-gcn,ResGCN,dynamic_gcn}, where the raw skeleton sequences are first transformed into either grid-structured or graph-structured formats (e.g.,pseudo-images and graph) and then to be fed into different models (e.g., CNNs and GCNs).


%TBC


% A milestone of GCN-based method is ST-GCN\cite{st-gcn}, which first constructs a sparse connected \textbf{undirected} spatial-temporal skeleton graph and then model the spatial and temporal dependencies in a factorised/alternative way. Since then, many variants of ST-GCN are proposed.  Some works focus on improving the spatial-temporal graph topology, for example, \cite{2s-agcn,ms-aagcn,dynamic_gcn} make the spatial graph connections learnable, \cite{dgcn} constructs a directed graph, \cite{ms-g3d} constructs a multi-scale spatial-graph and together with unified pathways for robust spatial-temporal information aggregation. 
% Other works such as \cite{shift-gcn} introduce the shift convolution in graph-structured data and \cite{ResGCN} introduce a novel residual bottleneck structures to make the model more efficient. And also, \cite{zhang2020context} explores contextual information between joints\cite{zhang2020context}. \cite{mst-gcn} efficiently expands the receptive filed to long-range in spatial-temporal domain.

% \textbf{However, most of the recent works focus on spatial modeling to generate better semantic representation of human skeleton, but paid less attention on temporal modeling of dynamic frames, which is crucial to action recognition. Specifically, 
% recent SOTA methods \cite{ms-g3d,ms-aagcn,MST-GCN} capture temporal context by utilizing multiple temporal (dilated) convolutions in its 2D or 3D blocks.}



% % The key to recognize actions from skeleton sequences is to encode robust short-range and long-range temporal dependencies
%  {\color{blue}{
% %  \textbf{Motivation}
 
% A key point in skeleton-based recognition is to robustly encode spatial correlations together with  temporal motion context in the feature representations. 
% Some fine-grained actions, such as  "writing" and "typing", need model to pay more attention on fine-grained temporal dynamics while some coarse-grained actions (e.g., fall, sit down) don't need such detailed information for recognition. 
% However, most of the existing works focus on using a single model to capture holistic motion patterns for various actions. It is relatively inefficient to capture temporal coarse-level and fine-level patterns simultaneously with a bundled kernels and in some cases, such architecture suffers from recognizing fine-grained actions such as "writing" and "typing".
% As shown in Figure xxx \ref{Fig.Ads}, to remedy/alleviate the above drawbacks, we propose a dual head architecture which can effectively learn a  robust representations of the input skeleton sequences from coarse-level and fine-level.  


% Our network consists of three modules: a backbone module extracts low level spatial and temporal features; a coarse-and-fine dual head module to encode motion patterns from two temporal perspectives;  a cross-head communication module used for two heads to help each other and enhance the representations of two heads mutually; a late-fusion module for coarse-fine combination
% Specifically,  we adopt the basic Spatial-Temporal Graph Convolution block (STGC-block) in previous work \cite{ms-g3d} as our backbone module. Such basic blocks are also used in other part.
% In our fine head, multiple STGC-blocks are concatenated to extract fine-grained motion contexts from the features with high temporal resolution. Meanwhile, in the coarse head, another bunch of STGC-blocks are concatenated to extract coarse-grained motion dependencies at the down-sampled temporal resolution. 
% To further improve the cross head context fusion and facilitate the representation modeling, we propose a cross-head communication module which contains a temporal attention block and a spatial attention block. Temporal attention block takes the feature maps from fine head to estimate a temporal attention, indicating the importance of each frame which is then utilized to re-weight the features in the coarse head in temporal dimension. Spatial attention block takes the feature maps from coarse head to estimate a spatial attention, indicating the importance of each joint.  The spatial attention is shared in all frames, and passes relative robust spatial contexts from coarse head to fine head. Such cross head temporal attention and spatial attention is alternately performed through forward process of dual heads, achieving efficient spatial and temporal dependency modeling. 
% In the end, each head predicts a probability of each action class, and we fuse the estimated scores to generate final predictions. 


% Specifically,  we adopt the basic Spatial-Temporal Graph Convolution block (STGC-block) in previous work \cite{ms-g3d} as our backbone module. A fine head extracts features at a high temporal resolution, and a coarse head extracts features at low temporal resolution. 
%  During forward process, the fine head focuses on extracting fine-grained temporal contexts, and simultaneously, the coarse head focuses on capturing coarse-grained temporal dependencies. An alternative cross-head communication mechanism is designed for mutually enhancing feature representations by leveraging their individual advantages. (Finer Temporal Attention of fine head  and stronger Spatial Attention of Coarse head). 


% To achieve this, we propose a coarse-fine dual head network. Our network consists of three modules: a backbone module extracts low level spatial and temporal features; a coarse-fine dual head module to encode both short-term and long-term dependencies; and a voting module to aggregates the short-term information and long-term information via score level fusion. We adopt the basic GCN block in previous work \cite{ms-g3d} as our backbone module. Our coarse-fine dual head module consists of a fine head and a coarse to model short-term and long-term dependencies. Specifically, in our fine head, multiple GCN blocks are concatenated to extract fine-grained motion contexts from the features with high temporal resolution. Meanwhile, in the coarse head, another bunch of GCN blocks are concatenated to extract long range motion dependencies at the down-sampled temporal resolution. To further improve the cross head context fusion and facilitate long range dependency modeling, we propose a cross head temporal attention block, which takes the feature maps from fine head to estimate a temporal attention, indicating the importance of each frame. The temporal attention is then utilized to re-weight the features in the coarse head. Moreover, we propose a cross head spatial attention mechanism, which takes the feature maps from coarse head to estimate a spatial attention, indicating the importance of each joint. The spatial attention is shared in all frames, and passes long range contexts from coarse head to fine head, to enhance fine representations. Such cross head temporal attention and spatial attention is alternately performed though forward process of dual heads, achieving efficient short-term and long-term dependency modeling. In the last stage, our voting module first predicts the action scores via each head, and then fuses the predictions via weighted sum. 

% We adopt the basic Spatial-Temporal Graph Convolution block (STGC-block) in previous work \cite{ms-g3d} as our backbone module. 
% To further improve the cross head context fusion and facilitate long range dependency modeling, we propose a cross head temporal attention block, which takes the feature maps from fine head to estimate a temporal attention, indicating the importance of each frame. The temporal attention is then utilized to re-weight the features in the coarse head. Moreover, we propose a cross head spatial attention mechanism, which takes the feature maps from coarse head to estimate a spatial attention, indicating the importance of each joint. The spatial attention is shared in all frames, and passes long range contexts from coarse head to fine head, to enhance fine representations.

% }}



% \vspace{5cm}
% The key to recognize actions from skeleton sequences is to encode short-term and long-term temporal motion context in the feature representations. On the one hand, many actions are discriminative by subtle temporal movements of pivotal key points; on the other hand, long range dependency in temporal dimension is crucial for action recognition. Existing works address the problem by concatenating multiple dilated temporal convolutions and 3D graph blocks with multiple window sizes\cite{ms-g3d,MST-GCN}. Despite the promising performance they achieve, there still exist several drawbacks in the design of their architectures. Specifically, in MS-G3D, the factorized pathway and G3D blocks have different temporal kernel sizes/receptive fields, hence that each graph node receives more messages from nearby nodes than long distant nodes. As a result, the aggregating process is biased to short-range dependency. Similarly in MST-GCN, long range contexts is estimated based on short range contexts. In addition, the short range and long range temporal context are mixed in their representation, hence the features will encode more local information than long range contexts due to biased aggregation.

% \textbf{To sufficiently capture long range dependencies,} we propose a dual head framework to remedy the above drawbacks. Our key idea is to sub-sample the frames at temporal dimension to maintain an additional coarse branch. Since we have reduced the frame rate, the adjacent feature frames are actually long range in their original temporal resolution. Due to sub-sampling process, we have removed the fine-grained temporal motion contexts and hence the network will focus on long range modeling. 

% Specifically, our framework has two heads: a fine head extracts features at a high temporal resolution, and a coarse head extracts features at low temporal resolution. During forward process, the fine head focuses on extracting fine-grained temporal contexts, and parallel the coarse head focuses on long range temporal dependencies. In the end, each head predicts a probability of each action class, and we fuse the estimated scores to generate final predictions. 

% To achieve this, we propose a coarse-fine dual head network. Our network consists of three modules: a backbone module extracts low level spatial and temporal features; a coarse-fine dual head module to encode both short-term and long-term dependencies; and a voting module to aggregates the short-term information and long-term information via score level fusion. We adopt the basic GCN block in previous work \cite{ms-g3d} as our backbone module. Our coarse-fine dual head module consists of a fine head and a coarse to model short-term and long-term dependencies. Specifically, in our fine head, multiple GCN blocks are concatenated to extract fine-grained motion contexts from the features with high temporal resolution. Meanwhile, in the coarse head, another bunch of GCN blocks are concatenated to extract long range motion dependencies at the down-sampled temporal resolution. To further improve the cross head context fusion and facilitate long range dependency modeling, we propose a cross head temporal attention block, which takes the feature maps from fine head to estimate a temporal attention, indicating the importance of each frame. The temporal attention is then utilized to re-weight the features in the coarse head. Moreover, we propose a cross head spatial attention mechanism, which takes the feature maps from coarse head to estimate a spatial attention, indicating the importance of each joint. The spatial attention is shared in all frames, and passes long range contexts from coarse head to fine head, to enhance fine representations. Such cross head temporal attention and spatial attention is alternately performed though forward process of dual heads, achieving efficient short-term and long-term dependency modeling. In the last stage, our voting module first predicts the action scores via each head, and then fuses the predictions via weighted sum. 




%现在的方法，MS-G3D，同时考虑了short range和long range的dependency，在每一个block里，利用了mutliple dilated convolutions with different dilation rates, and multiple G3D components with different window sizes to capture both short range and long range dependency. However, is this blocks, long range dependency is not sufficiently modeled like short-range, since that times of short range message passing is much more than long range message passing. It makes the network 
% In this work, we propose a novel approach to skeleton-based action recognition in order to perform spatial and temporal modeling in an effective way. Our key idea is to utilize two branches of networks, one branch focuses on extracting joint-level semantic features, and the other branch focuses on extracting detailed temporal motion information. In the end, we are able to fuse the outputs of both networks, performing joint spatial and temporal inference. 

% {
% \color{blue} Motivation 

% %粗细粒度的结合在Action Recognition中的作用
% % 1. 粗粒度的网络如何从粗粒度的动作中提取 coarse-grained feature
% % 2. 细粒度网络如何识从细粒度的动作中提取 fine-grained feature
% % 3. 为什么要两者结合
% Modelling robust temporal dependencies from various skeleton sequences is a fundamental challenge in skeleton-based action recognition. Most existing methods often overlook the hierarchical granularities of actions in time domain and thus fail to extract discriminative representations for fine-grained actions (eg. reading, writing and eating food). 
% (or modelling discriminative dependencies for different action granularities in temporal dimension)
% In this paper, we propose a novel attention-enhanced cross-fine dual head networks (C2F-DH Net)for robust temporal modelling by exploring different action granularities. 

% Our C2F-DH Net consists of three main stages:

% 1) We first construct A coarse representation net (CRN) to model long-range temporal dependencies, A Fine context proposal net (FCPN) which can  produce finer context information. 

% 2) Then we apply a cross-branch attention mechanism between the two branches. The fine head can refine coarse head by producing finer temporal context, while the coarse head can in turn provide fine head with coarse spatial configuration information. Finally, these two branches can refine each other along with the model optimization process. 

% 3) Finally, a  voting mechanism is adopted aims at taking the most advantages of these two different granularities of representations. This voting mechanism is accompanied with two losses, thus our model can learn the fine-grained features and coarse-grained features individually along with the optimization process of the model. The final voting results of two heads is thus robust both for  fine-level and coarse-level inputs.

% % }
% \vspace{4cm}
% To achieve this, we first utilize a GCN block \cite{ms-g3d} to generate features of input skeleton sequence, and then propose a dual head network based on the backbone feature extractor, where each head is associated with spatial or temporal modeling. The spatial head aims at extracting semantic features between different joints while ignoring fine-grained temporal context, and the temporal head explores finer temporal motions while weakening spatial dependencies. To this end, we adopt two slightly different modification from the basic GCN block \cite{ms-g3d}. In the spatial head, we down sample the feature maps in temporal dimension, the latter computations are based on the resulting features. In addition, we reduce the kernel sizes and dilation rates of the temporal convolutions. In this way the feature maps carry coarse temporal motion context, and hence our network can focus more on spatial modeling. As for the temporal head, we borrow the idea of the SlowFast Network\cite{slowfast}, which decreases the dimensions of feature channels. In skeletal data, each joint has its semantic meaning, hence the joint positional data are naturally aligned in different temporal frames. Extracting temporal movements of the same joint or nearby joints in different frames is much easier than extracting abstract spatial features, hence reducing feature channels can enforce the network encode less spatial context but focus on temporal motions. To sufficient exploit our spatial head and temporal head, we further propose a novel attention mechanism to enhance the spatial and temporal features. Finally, each head generates a probabilistic prediction of action classes. The final prediction is generated by combing the voting of both heads.

% Specifically, the spatial head consists of a sub-sampling layer followed by two modified GCN blocks and a prediction layer. The subsampling layer is used to downsample feature maps at temporal resolution. For the GCN structure, we decrease the number of G3D pathways in MS-G3D, aiming to weaken the 3D or temporal modeling. We also decrease the dilation rates and kernel sizes of the temporal convolution blocks or G3D blocks. The temporal head consists of an embedding layer to decrease feature channels and two MS-G3D blocks, and a prediction layers. To further enhance the learned temporal and spatial context, we propose a cross head attention mechanism, which utilizes the spatial head to estimates an spatial joint-level attention for each joint and the temporal head to estimate the temporal attention of each temporal frame. The estimated attentions are used to enhance spatial or temporal features of the other bead in a residual way. Finally, the predictions of both heads are used to voting for final prediction.

% \textcolor{blue}{I'm not sure whether should remain this or move it to section 2:} Our method is different from the SlowFast Network\cite{slowfast}. First of all, we generate the slow branch by subsampling the feature maps instead of raw data frames. Such structure is more like the Temporal Pyramid Network\cite{tpn} or HRNet\cite{hrnet}. In addition, our final prediction is generated by voting of both heads, instead of the fusion of each head's feature maps. We will describe the related work in detail in the next section. \textcolor{red}{By modifying the G3D blocks, our network has fewer parameters than MS-G3D.}.




\begin{figure*}[t]
	\centering
	\includegraphics[width=1.\textwidth]{paperSec/imgs/Overview_Framework_Version3.pdf}
	\caption{Overview of our proposed framework. We first utilize a STGC block to generate backbone features of skeleton data, and then use a coarse head to capture coarse grained motion patterns, a fine head to encode fine-grained subtle temporal movements. Cross head spatial and temporal attentions are exploited to mutually enhance  feature representations. Finally each head generates a probabilistic prediction of actions and the ultimate estimation is given by fusion of both predictions.}
	\label{fig:Overall_Framework}
\end{figure*}


==> paperSec/intro.tex <==

\section{Introduction}

Action recognition is a fundamental task in human-centered scene understanding and has achieved much progress in computer vision and multimedia. Recently, skeleton-based action recognition has attracted increasing attention to the community due to the advent of inexpensive motion sensors \cite{cao2018openpose,ntu_60} and effective human pose estimation algorithms \cite{st-gcn,2s-agcn,ms-g3d}. The skeleton data typically are more compact and robust to environment conditions than its video counterpart, and accurate action recognition from skeletons can greatly benefit a wide range of applications, such as human-computer interactions, healthcare assistance and physical education. 


%\vspace{5cm}
Different from RGB videos, skeleton data contain only the 2D or 3D coordinates of human joints, which makes skeleton-based action recognition particularly challenging due to the lack of image-based contextual information.
In order to capture discriminative spatial structure and temporal motion patterns, existing methods \cite{ms-aagcn,st-gcn,ms-g3d} usually rely on a unified spatio-temporal representation of the skeleton data at the original frame rate of input sequence. While such a strategy may have the capacity to capture action patterns of multiple scales, they often suffer from inaccurate predictions on fine-grained action classes due to model complexity and limited training data. To tackle this problem, we argue that a more effective solution is to explicitly model the motion patterns of skeleton sequences at multiple temporal granularity.  
For example, actions such as `sit down' or `stand up' can be distinguished based on coarse-grained motion patterns, while recognizing actions like `put on a shoe' or `take off a shoe' requires understanding not only coarse-grained motions but also subtle temporal movements of pivotal joints. To the best of our knowledge, such multiple granularity of temporal motion information remains implicit in the recent deep graph network-based approaches, which is less effective. 


%and hence is able to predict reasonable action probabilities from skeleton data despite the lack of image contexts. However, we argue that a skeleton sequence contains different granularities of temporal information and recognizing actions requires different granularities of motion patterns. 
%For example, we may first take a glimpse of a sequence to get a coarse understanding of the action, and then take into account to the finer grained motion patterns for further inference. 
%To the best of our knowledge, such different granurities of temporal motion information are not sufficient explored in recent GCN based networks. Prior GCN based methods\cite{ms-aagcn,st-gcn,ms-g3d} couple different granularities of temporal motions in a unified representation, which is ineffective.

In this paper, we propose a dual-head graph neural network framework for skeleton-based action recognition in order to capture both coarse-grained and fine-grained motion patterns. Our key idea is to utilize two branches of interleaved graph networks to extract features at two different temporal resolutions. The branch with lower temporal resolution captures motion patterns at a coarse level, while
the branch with higher temporal resolution is able to encode more subtle temporal movements. Such coarse-level and fine-level feature extraction are processed in parallel and finally the outputs of both branches are fused to perform dual-granularity action classification.

Specifically, we first exact a base feature representation of the input skeleton sequence by feeding it into a backbone Graph Convolution Network (GCN). 
The backbone network extracts low level spatial and temporal features. Then we perform two different operations to the resulting feature maps: in one operation we subsample the feature maps at temporal dimension with a downsampling rate, such operation removes the detailed motion information and hence produces a coarse grained representation; in the other operation we utilize an identity mapping to get a fine grained representation. 
\begin{figure}[tbp]
	\includegraphics[width=0.4\textwidth]{paperSec/imgs/ad1.pdf}
	\caption{Some actions can be recognized via coarse grained temporal motion patterns(first sample), while recognizing other actions requires not only coarse grained motion but subtle temporal movements(second sample).}
	\vspace{-0.5cm}
	\label{fig:advertisment}
\end{figure}

To achieve this, we utilize two types of GCN blocks to process the resulting coarse-grained and fine-grained representations, which are referred as \textit{fine head} and \textit{coarse head}. Each head consists of two GCN blocks, which iteratively extract features with respective granularity. Our coarse head captures the correlations between joints at lower temporal resolution, hence infers actions in a more holistic way. To facilitate such coarse level inference, we utilize the fine grained feature representation in fine head to estimate a temporal attention, which indicates the importance of each frame. The temporal attention is utilized to re-weight the features at coarse head. The intuition behind such cross head attention is simple: we pass the fine-grained motion contexts encoded in the attention to coarse head to remedy the lack of fine level information in coarse head. Similarly, we utilize the coarse grained features to estimate a spatial attention indicating the joint level importance. The spatial attention is utilized to highlight the pivotal joint nodes in fine head. Our fine GCN blocks are able to focus on the subtle temporal movements of the pivotal joints and hence extract the fine-grained information effectively. 

Moreover, our dual granularity head consists of two stages. At each stage, a fine GCN block extracts fine grained features at higher temporal resolution, and then generates a temporal attention based on its resulting feature map. Then our coarse head re-weights the coarse level feature with the temporal attention, and further utilizes a coarse GCN block to perform coarse level inference. At last, we predict a joint level spatial attention based on the coarse representation, which is used to enhance fine grained features by re-weighting. Such processes are alternately processed in each stage. Finally, each head predicts an action score, and the final prediction is given by fusion of two scores.

We conduct the experiments on three public datasets: NTU-60, NTU-120, Kinetics-Skeleton. As a result, our method outperforms existing works in all benchmarks, achieving new state-of-the-art, demonstrating the effectiveness of the proposed coarse-and-fine dual head structure. To summarize, our contributions are three-folds:

% 1). propose a dual head network that two heads are slightly different in temporal resolution or channel 
% dimensions, aiming to joint capture spatial and temporal context effectively;

% 2). propose a cross branch attention mechanism to enhance the spatial and temporal features of both heads, the attentions are used for fusing information of two heads. \textcolor{blue}{Alternating strategy}

% 2). propose a voting mechanism to skeleton-based action recognition, which simply fuses the predictions of both heads. 

% 4). achieve new state-of-the-art on three public benchmarks.

1) We propose a dual head architecture which can effectively learn robust representations from temporal coarse-level and fine-level for skeleton sequence data.

2) We propose a cross head attention mechanism to mutually enhance the features of both heads in an alternative manner. 

3) Our dual-head graph neural network achieves new state-of-the-art on three public benchmarks.




% Specifically, each stage consists of three steps. At step one, a fine GCN block first processes the fine grained representation, and then estimates a temporal attention based on resulting fine features. The temporal attention indicates the importance of each frame, which is used to re-weight the features in coarse head. At step two, a coarse GCN block updates coarse feature and estimate a spatial attention based on the resulting coarse representation, which indicates the importance of each joint. At step three, the fine grained feature is re-weighted by the spatial attention from coarse head. The intuition 



% \vspace{5cm}

%Our key idea is to sub-sample the frames at temporal dimension to maintain an additional coarse branch. Since we have reduced the frame rate, the adjacent feature frames are actually long range in their original temporal resolution. Due to sub-sampling process, we have removed the fine-grained temporal motion contexts and hence the network will focus on long range modeling. 

% To achieve this, we propose a coarse-fine dual head network. Our network consists of three modules: a backbone module extracts low level spatial and temporal features; a coarse-fine dual head module to encode both short-term and long-term dependencies; and a voting module to aggregates the short-term information and long-term information via score level fusion. We adopt the basic GCN block in previous work \cite{ms-g3d} as our backbone module. Our coarse-fine dual head module consists of a fine head and a coarse to model short-term and long-term dependencies. Specifically, in our fine head, multiple GCN blocks are concatenated to extract fine-grained motion contexts from the features with high temporal resolution. Meanwhile, in the coarse head, another bunch of GCN blocks are concatenated to extract long range motion dependencies at the down-sampled temporal resolution. To further improve the cross head context fusion and facilitate long range dependency modeling, we propose a cross head temporal attention block, which takes the feature maps from fine head to estimate a temporal attention, indicating the importance of each frame. The temporal attention is then utilized to re-weight the features in the coarse head. Moreover, we propose a cross head spatial attention mechanism, which takes the feature maps from coarse head to estimate a spatial attention, indicating the importance of each joint. The spatial attention is shared in all frames, and passes long range contexts from coarse head to fine head, to enhance fine representations. Such cross head temporal attention and spatial attention is alternately performed though forward process of dual heads, achieving efficient short-term and long-term dependency modeling. In the last stage, our voting module first predicts the action scores via each head, and then fuses the predictions via weighted sum. 





%Understanding actions from a skeleton sequence reuqires different granularities of motion patterns, existing works encodes multiple grained motion information in a unified representation, which is inefficient. Our method captures coarse grained and fine grained motion patterns in two different heads, hence is more robust to fine-grained action classes, e.g. 'reading' and 'writing'.



%\vspace{5cm}




%  Action recognition is a fundamental problem in computer vision. Recently, skeleton-based action recognition have attracted increasing attention due to the light-weight data source, high-level semantic information and robustness against complicated environment\cite{st-gcn,2s-agcn,ms-g3d}.  (Wang et al. 2018; Vemulapalli, Arrate, andChellappa 2014; Liu, Liu, and Chen 2017; Tu, Liu, and Liu2018). 
 
%  The advent of cheap motion sensors \cite{kinect,ntu_60} and effective human pose estimation algorithms  \cite{st-gcn,2s-agcn,ms-g3d} further speed up this research topic. 
%  Accurately recognizing actions from skeletal data can be very helpful in human-computer interactions, healthcare assistance and physical education\cite{xxx}. 

% related work
% Different from RGB videos, skeleton data only contains the 2D or 3D coordinates of the human key joints and lacks of image level contextual information. Hence our designed model should focus on the structure of human and motion patterns of skeletal joints. This causes the task of skeleton-based action recognition very challenging. 
% Existing works mainly focus on extracting discriminative spatial and temporal features of skeletal joints \cite{ms-aagcn,st-gcn}. Recent deep network based methods can be categorized into three types: RNNs, CNNs and GCNs. First of all, a typical method of skeleton based action recognition is RNNs\cite{xx}. Those methods first extract frame level skeletal features with a feature extractor and then modeling sequential dependencies with RNN models\cite{xx}. Typical drawback of those methods is that they compress the joint data to person-level feature in each frame and hence the intra-joint dependencies in temporal domain are hard to capture \cite{st-gcn}. The second pipeline for skeleton-based action recognition can be summarized as CNNs\cite{xxx}, which treat the joint positional data as pixels. They first flatten skeletal data of each frame to a column of pixels and then stack multiple frame data to generate an pesudo-image. Finally image-based classification CNNs are used for action recognition. However, as human skeletons lie in a non-Euclidean space, directly stacking different joints together and utilizing convolution operations may not be effective in modeling joint-level dependencies. The third framework of our task is GCNs\cite{st-gcn}, which are widely adopted in recent years due to their efficacy in spatial and temporal modeling. A milestone of GCN-based method is ST-GCN\cite{st-gcn}, which defines a sparse connected spatial-temporal graph that both considers human natural structure and temporal motion dependencies in space-time domain. Since then, many works attempted to improve the graph topology by making the graph connections learnable\cite{2s-agcn, dynamic_gcn}, adding residual layers\cite{ResGCN},  exploring contextual information between joints\cite{zhang2020context}, or introducing multi-scale spatial connections\cite{ms-g3d}.  


%allowing action recognition models to focus on understanding the action itself.
% For example, we can not infer which sport of a sport player is playing by his clothes or environments but only the skeletal sequence. This causes the task of skeleton-based action recognition very challenging. 

% In recent years, deep learning based methods have been the dominant stream for skeleton-based action recognition\cite{st-gcn, ms-aagcn,ms-g3d,decouple_gcn_cheng2020eccv,shift-gcn,ResGCN,dynamic_gcn}, where the raw skeleton sequences are first transformed into either grid-structured or graph-structured formats (e.g.,pseudo-images and graph) and then to be fed into different models (e.g., CNNs and GCNs).


%TBC


% A milestone of GCN-based method is ST-GCN\cite{st-gcn}, which first constructs a sparse connected \textbf{undirected} spatial-temporal skeleton graph and then model the spatial and temporal dependencies in a factorised/alternative way. Since then, many variants of ST-GCN are proposed.  Some works focus on improving the spatial-temporal graph topology, for example, \cite{2s-agcn,ms-aagcn,dynamic_gcn} make the spatial graph connections learnable, \cite{dgcn} constructs a directed graph, \cite{ms-g3d} constructs a multi-scale spatial-graph and together with unified pathways for robust spatial-temporal information aggregation. 
% Other works such as \cite{shift-gcn} introduce the shift convolution in graph-structured data and \cite{ResGCN} introduce a novel residual bottleneck structures to make the model more efficient. And also, \cite{zhang2020context} explores contextual information between joints\cite{zhang2020context}. \cite{mst-gcn} efficiently expands the receptive filed to long-range in spatial-temporal domain.

% \textbf{However, most of the recent works focus on spatial modeling to generate better semantic representation of human skeleton, but paid less attention on temporal modeling of dynamic frames, which is crucial to action recognition. Specifically, 
% recent SOTA methods \cite{ms-g3d,ms-aagcn,MST-GCN} capture temporal context by utilizing multiple temporal (dilated) convolutions in its 2D or 3D blocks.}



% % The key to recognize actions from skeleton sequences is to encode robust short-range and long-range temporal dependencies
%  {\color{blue}{
% %  \textbf{Motivation}
 
% A key point in skeleton-based recognition is to robustly encode spatial correlations together with  temporal motion context in the feature representations. 
% Some fine-grained actions, such as  "writing" and "typing", need model to pay more attention on fine-grained temporal dynamics while some coarse-grained actions (e.g., fall, sit down) don't need such detailed information for recognition. 
% However, most of the existing works focus on using a single model to capture holistic motion patterns for various actions. It is relatively inefficient to capture temporal coarse-level and fine-level patterns simultaneously with a bundled kernels and in some cases, such architecture suffers from recognizing fine-grained actions such as "writing" and "typing".
% As shown in Figure xxx \ref{Fig.Ads}, to remedy/alleviate the above drawbacks, we propose a dual head architecture which can effectively learn a  robust representations of the input skeleton sequences from coarse-level and fine-level.  


% Our network consists of three modules: a backbone module extracts low level spatial and temporal features; a coarse-and-fine dual head module to encode motion patterns from two temporal perspectives;  a cross-head communication module used for two heads to help each other and enhance the representations of two heads mutually; a late-fusion module for coarse-fine combination
% Specifically,  we adopt the basic Spatial-Temporal Graph Convolution block (STGC-block) in previous work \cite{ms-g3d} as our backbone module. Such basic blocks are also used in other part.
% In our fine head, multiple STGC-blocks are concatenated to extract fine-grained motion contexts from the features with high temporal resolution. Meanwhile, in the coarse head, another bunch of STGC-blocks are concatenated to extract coarse-grained motion dependencies at the down-sampled temporal resolution. 
% To further improve the cross head context fusion and facilitate the representation modeling, we propose a cross-head communication module which contains a temporal attention block and a spatial attention block. Temporal attention block takes the feature maps from fine head to estimate a temporal attention, indicating the importance of each frame which is then utilized to re-weight the features in the coarse head in temporal dimension. Spatial attention block takes the feature maps from coarse head to estimate a spatial attention, indicating the importance of each joint.  The spatial attention is shared in all frames, and passes relative robust spatial contexts from coarse head to fine head. Such cross head temporal attention and spatial attention is alternately performed through forward process of dual heads, achieving efficient spatial and temporal dependency modeling. 
% In the end, each head predicts a probability of each action class, and we fuse the estimated scores to generate final predictions. 


% Specifically,  we adopt the basic Spatial-Temporal Graph Convolution block (STGC-block) in previous work \cite{ms-g3d} as our backbone module. A fine head extracts features at a high temporal resolution, and a coarse head extracts features at low temporal resolution. 
%  During forward process, the fine head focuses on extracting fine-grained temporal contexts, and simultaneously, the coarse head focuses on capturing coarse-grained temporal dependencies. An alternative cross-head communication mechanism is designed for mutually enhancing feature representations by leveraging their individual advantages. (Finer Temporal Attention of fine head  and stronger Spatial Attention of Coarse head). 


% To achieve this, we propose a coarse-fine dual head network. Our network consists of three modules: a backbone module extracts low level spatial and temporal features; a coarse-fine dual head module to encode both short-term and long-term dependencies; and a voting module to aggregates the short-term information and long-term information via score level fusion. We adopt the basic GCN block in previous work \cite{ms-g3d} as our backbone module. Our coarse-fine dual head module consists of a fine head and a coarse to model short-term and long-term dependencies. Specifically, in our fine head, multiple GCN blocks are concatenated to extract fine-grained motion contexts from the features with high temporal resolution. Meanwhile, in the coarse head, another bunch of GCN blocks are concatenated to extract long range motion dependencies at the down-sampled temporal resolution. To further improve the cross head context fusion and facilitate long range dependency modeling, we propose a cross head temporal attention block, which takes the feature maps from fine head to estimate a temporal attention, indicating the importance of each frame. The temporal attention is then utilized to re-weight the features in the coarse head. Moreover, we propose a cross head spatial attention mechanism, which takes the feature maps from coarse head to estimate a spatial attention, indicating the importance of each joint. The spatial attention is shared in all frames, and passes long range contexts from coarse head to fine head, to enhance fine representations. Such cross head temporal attention and spatial attention is alternately performed though forward process of dual heads, achieving efficient short-term and long-term dependency modeling. In the last stage, our voting module first predicts the action scores via each head, and then fuses the predictions via weighted sum. 

% We adopt the basic Spatial-Temporal Graph Convolution block (STGC-block) in previous work \cite{ms-g3d} as our backbone module. 
% To further improve the cross head context fusion and facilitate long range dependency modeling, we propose a cross head temporal attention block, which takes the feature maps from fine head to estimate a temporal attention, indicating the importance of each frame. The temporal attention is then utilized to re-weight the features in the coarse head. Moreover, we propose a cross head spatial attention mechanism, which takes the feature maps from coarse head to estimate a spatial attention, indicating the importance of each joint. The spatial attention is shared in all frames, and passes long range contexts from coarse head to fine head, to enhance fine representations.

% }}



% \vspace{5cm}
% The key to recognize actions from skeleton sequences is to encode short-term and long-term temporal motion context in the feature representations. On the one hand, many actions are discriminative by subtle temporal movements of pivotal key points; on the other hand, long range dependency in temporal dimension is crucial for action recognition. Existing works address the problem by concatenating multiple dilated temporal convolutions and 3D graph blocks with multiple window sizes\cite{ms-g3d,MST-GCN}. Despite the promising performance they achieve, there still exist several drawbacks in the design of their architectures. Specifically, in MS-G3D, the factorized pathway and G3D blocks have different temporal kernel sizes/receptive fields, hence that each graph node receives more messages from nearby nodes than long distant nodes. As a result, the aggregating process is biased to short-range dependency. Similarly in MST-GCN, long range contexts is estimated based on short range contexts. In addition, the short range and long range temporal context are mixed in their representation, hence the features will encode more local information than long range contexts due to biased aggregation.

% \textbf{To sufficiently capture long range dependencies,} we propose a dual head framework to remedy the above drawbacks. Our key idea is to sub-sample the frames at temporal dimension to maintain an additional coarse branch. Since we have reduced the frame rate, the adjacent feature frames are actually long range in their original temporal resolution. Due to sub-sampling process, we have removed the fine-grained temporal motion contexts and hence the network will focus on long range modeling. 

% Specifically, our framework has two heads: a fine head extracts features at a high temporal resolution, and a coarse head extracts features at low temporal resolution. During forward process, the fine head focuses on extracting fine-grained temporal contexts, and parallel the coarse head focuses on long range temporal dependencies. In the end, each head predicts a probability of each action class, and we fuse the estimated scores to generate final predictions. 

% To achieve this, we propose a coarse-fine dual head network. Our network consists of three modules: a backbone module extracts low level spatial and temporal features; a coarse-fine dual head module to encode both short-term and long-term dependencies; and a voting module to aggregates the short-term information and long-term information via score level fusion. We adopt the basic GCN block in previous work \cite{ms-g3d} as our backbone module. Our coarse-fine dual head module consists of a fine head and a coarse to model short-term and long-term dependencies. Specifically, in our fine head, multiple GCN blocks are concatenated to extract fine-grained motion contexts from the features with high temporal resolution. Meanwhile, in the coarse head, another bunch of GCN blocks are concatenated to extract long range motion dependencies at the down-sampled temporal resolution. To further improve the cross head context fusion and facilitate long range dependency modeling, we propose a cross head temporal attention block, which takes the feature maps from fine head to estimate a temporal attention, indicating the importance of each frame. The temporal attention is then utilized to re-weight the features in the coarse head. Moreover, we propose a cross head spatial attention mechanism, which takes the feature maps from coarse head to estimate a spatial attention, indicating the importance of each joint. The spatial attention is shared in all frames, and passes long range contexts from coarse head to fine head, to enhance fine representations. Such cross head temporal attention and spatial attention is alternately performed though forward process of dual heads, achieving efficient short-term and long-term dependency modeling. In the last stage, our voting module first predicts the action scores via each head, and then fuses the predictions via weighted sum. 




%现在的方法，MS-G3D，同时考虑了short range和long range的dependency，在每一个block里，利用了mutliple dilated convolutions with different dilation rates, and multiple G3D components with different window sizes to capture both short range and long range dependency. However, is this blocks, long range dependency is not sufficiently modeled like short-range, since that times of short range message passing is much more than long range message passing. It makes the network 
% In this work, we propose a novel approach to skeleton-based action recognition in order to perform spatial and temporal modeling in an effective way. Our key idea is to utilize two branches of networks, one branch focuses on extracting joint-level semantic features, and the other branch focuses on extracting detailed temporal motion information. In the end, we are able to fuse the outputs of both networks, performing joint spatial and temporal inference. 

% {
% \color{blue} Motivation 

% %粗细粒度的结合在Action Recognition中的作用
% % 1. 粗粒度的网络如何从粗粒度的动作中提取 coarse-grained feature
% % 2. 细粒度网络如何识从细粒度的动作中提取 fine-grained feature
% % 3. 为什么要两者结合
% Modelling robust temporal dependencies from various skeleton sequences is a fundamental challenge in skeleton-based action recognition. Most existing methods often overlook the hierarchical granularities of actions in time domain and thus fail to extract discriminative representations for fine-grained actions (eg. reading, writing and eating food). 
% (or modelling discriminative dependencies for different action granularities in temporal dimension)
% In this paper, we propose a novel attention-enhanced cross-fine dual head networks (C2F-DH Net)for robust temporal modelling by exploring different action granularities. 

% Our C2F-DH Net consists of three main stages:

% 1) We first construct A coarse representation net (CRN) to model long-range temporal dependencies, A Fine context proposal net (FCPN) which can  produce finer context information. 

% 2) Then we apply a cross-branch attention mechanism between the two branches. The fine head can refine coarse head by producing finer temporal context, while the coarse head can in turn provide fine head with coarse spatial configuration information. Finally, these two branches can refine each other along with the model optimization process. 

% 3) Finally, a  voting mechanism is adopted aims at taking the most advantages of these two different granularities of representations. This voting mechanism is accompanied with two losses, thus our model can learn the fine-grained features and coarse-grained features individually along with the optimization process of the model. The final voting results of two heads is thus robust both for  fine-level and coarse-level inputs.

% % }
% \vspace{4cm}
% To achieve this, we first utilize a GCN block \cite{ms-g3d} to generate features of input skeleton sequence, and then propose a dual head network based on the backbone feature extractor, where each head is associated with spatial or temporal modeling. The spatial head aims at extracting semantic features between different joints while ignoring fine-grained temporal context, and the temporal head explores finer temporal motions while weakening spatial dependencies. To this end, we adopt two slightly different modification from the basic GCN block \cite{ms-g3d}. In the spatial head, we down sample the feature maps in temporal dimension, the latter computations are based on the resulting features. In addition, we reduce the kernel sizes and dilation rates of the temporal convolutions. In this way the feature maps carry coarse temporal motion context, and hence our network can focus more on spatial modeling. As for the temporal head, we borrow the idea of the SlowFast Network\cite{slowfast}, which decreases the dimensions of feature channels. In skeletal data, each joint has its semantic meaning, hence the joint positional data are naturally aligned in different temporal frames. Extracting temporal movements of the same joint or nearby joints in different frames is much easier than extracting abstract spatial features, hence reducing feature channels can enforce the network encode less spatial context but focus on temporal motions. To sufficient exploit our spatial head and temporal head, we further propose a novel attention mechanism to enhance the spatial and temporal features. Finally, each head generates a probabilistic prediction of action classes. The final prediction is generated by combing the voting of both heads.

% Specifically, the spatial head consists of a sub-sampling layer followed by two modified GCN blocks and a prediction layer. The subsampling layer is used to downsample feature maps at temporal resolution. For the GCN structure, we decrease the number of G3D pathways in MS-G3D, aiming to weaken the 3D or temporal modeling. We also decrease the dilation rates and kernel sizes of the temporal convolution blocks or G3D blocks. The temporal head consists of an embedding layer to decrease feature channels and two MS-G3D blocks, and a prediction layers. To further enhance the learned temporal and spatial context, we propose a cross head attention mechanism, which utilizes the spatial head to estimates an spatial joint-level attention for each joint and the temporal head to estimate the temporal attention of each temporal frame. The estimated attentions are used to enhance spatial or temporal features of the other bead in a residual way. Finally, the predictions of both heads are used to voting for final prediction.

% \textcolor{blue}{I'm not sure whether should remain this or move it to section 2:} Our method is different from the SlowFast Network\cite{slowfast}. First of all, we generate the slow branch by subsampling the feature maps instead of raw data frames. Such structure is more like the Temporal Pyramid Network\cite{tpn} or HRNet\cite{hrnet}. In addition, our final prediction is generated by voting of both heads, instead of the fusion of each head's feature maps. We will describe the related work in detail in the next section. \textcolor{red}{By modifying the G3D blocks, our network has fewer parameters than MS-G3D.}.




\begin{figure*}[t]
	\centering
	\includegraphics[width=1.\textwidth]{paperSec/imgs/Overview_Framework/Overview_Framework_finalize.pdf}
	\caption{Overview of our proposed framework. We first utilize a STGC block to generate backbone features of skeleton data, and then use a coarse head to capture coarse grained motion patterns, a fine head to encode fine-grained subtle temporal movements. Cross head spatial and temporal attentions are exploited to mutually enhance  feature representations. Finally each head generates a probabilistic prediction of actions and the ultimate estimation is given by fusion of both predictions.}
	\label{fig:Overall_Framework}
\end{figure*}



==> paperSec/intro_new.tex <==

\section{Introduction}

Action recognition is a fundamental problem in computer vision. Recently, skeleton-based action recognition has attracted increasing attention to the community due to the advent of cheap motion sensors \cite{cao2018openpose,ntu_60} and effective human pose estimation algorithms\cite{st-gcn,2s-agcn,ms-g3d}. Accurately recognizing actions from skeleton data can be very helpful in human-computer interactions, healthcare assistance or physical education. 


%\vspace{5cm}
Different from RGB videos, skeleton data only contains the 2D or 3D coordinates of the human joints and lack of image level contextual information. This causes the task of skeleton-based action recognition very challenging.
The key to skeleton-based action is to explore discriminative spatial structure and temporal motion patterns. Due to the lack of image level contexts, existing methods\cite{ms-aagcn,st-gcn,ms-g3d} usually sample the skeleton data at the original frame rate of skeleton sequence. In this way, the input data of the network carry sufficient fine-grained temporal motion information, and hence is able to predict reasonable action probabilities from skeleton data despite the lack of image contexts. However, we argue that a skeleton sequence contains different granularities of temporal information and recognizing actions requires different granularities of motion patterns. 
%For example, we may first take a glimpse of a sequence to get a coarse understanding of the action, and then take into account to the finer grained motion patterns for further inference. 
For example, actions such as 'hand waving' or 'clapping' can be recognized by coarse grained motion patterns without detailed temporal information, while recognizing actions like 'type on a keyboard' or 'writing' requires understanding not only coarse grained motion but subtle temporal movements of pivotal joints. To the best of our knowledge, such different granurities of temporal motion information are not sufficient explored in recent GCN based networks. Prior GCN based methods\cite{ms-aagcn,st-gcn,ms-g3d} couple different granularities of temporal motions in a unified representation, which is ineffective.

\begin{figure}[!tbp]
% 	\includegraphics[width=0.5\textwidth]{paperSec/imgs/ad_picture/Ad_picture.pdf}
	\includegraphics[width=0.5\textwidth]{paperSec/imgs/ad_picture/adv-desen2.png}
	\caption{Some actions can be recognized via coarse-grained temporal motion patterns, such as "hand waving" while recognizing other actions requires not only coarse grained motion but subtle temporal movements(second sample).}
	\label{fig:advertisment}
\end{figure}


In this paper, we propose a dual head framework in order to capture both coarse grained and fine grained motion contexts effectively. Our key idea is to utilize two branch of networks to extract features at two different temporal resolutions. The branch with lower temporal resolution captures motion patterns in a coarse level, while
the branch with higher temporal resolution is able to encode more subtle temporal movements. Such coarse level feature extraction and fine level feature extraction are parallelly processed and finally the outputs of both branches are fused to perform dual-granularity reasoning.

To achieve this, we first take all frames of skeleton sequence and feed it into a backbone GCN. The backbone network extracts low level spatial and temporal features. Then we perform two different operations to the resulting feature maps: in one operation we subsample the feature maps at temporal dimension with a downsampling rate, such operation removes the detailed motion information and hence produces a coarse grained representation; in the other operation we utilize an identity mapping to get a fine grained representation. Then we utilize two types of GCN blocks to process the resulting coarse grained and fine grained representations. 


Specifically, the two representations with different granularities are processed in two branches, which are referred as \textit{fine head} and \textit{coarse head}. Each head consists of two GCN blocks, which iteratively extract features with respective granularity. Our coarse head captures the correlations between joints at lower temporal resolution, hence infers actions in a more holistic way. To facilitate such coarse level inference, we utilize the fine grained feature representation in fine head to estimate a temporal attention, which indicates the importance of each frame. The temporal attention is utilized to re-weight the features at coarse head. The intuition behind such cross head attention is simple: we pass the fine-grained motion contexts encoded in the attention to coarse head to remedy the lack of fine level information in coarse head. Similarly, we utilize the coarse grained features to estimate a spatial attention indicating the joint level importance. The spatial attention is utilized to highlight the pivotal joint nodes in fine head. Our fine GCN blocks are able to focus on the subtle temporal movements of the pivotal joints and hence extract the fine-grained information effectively. 

Moreover, our dual granularity head consists of two stages. At each stage, a fine GCN block extracts fine grained features at higher temporal resolution, and then generates a temporal attention based on its resulting feature map. Then our coarse head re-weights the coarse level feature with the temporal attention, and further utilizes a coarse GCN block to perform coarse level inference. At last, we predict a joint level spatial attention based on the coarse representation, which is used to enhance fine grained features by re-weighting. Such processes are alternately processed in each stage. Finally, each head predicts an action score, and the final prediction is given by fusion of two scores.

We conduct the experiments on three public datasets: NTU-60, NTU-120, Kinetics-Skeleton. As a result, our method outperforms existing works in all benchmarks, achieving new state-of-the-art, demonstrating the effectiveness of the proposed coarse-and-fine dual head structure. To summarize our contributions, we:

% 1). propose a dual head network that two heads are slightly different in temporal resolution or channel 
% dimensions, aiming to joint capture spatial and temporal context effectively;

% 2). propose a cross branch attention mechanism to enhance the spatial and temporal features of both heads, the attentions are used for fusing information of two heads. \textcolor{blue}{Alternating strategy}

% 2). propose a voting mechanism to skeleton-based action recognition, which simply fuses the predictions of both heads. 

% 4). achieve new state-of-the-art on three public benchmarks.

1). propose a dual head architecture which can effectively learn robust representations from temporal coarse-level and fine-level for skeleton sequence data.

2). propose a cross head attention mechanism to mutually enhance the features of both heads in an alternative manner. 

3). achieve new state-of-the-art on three public benchmarks.




% Specifically, each stage consists of three steps. At step one, a fine GCN block first processes the fine grained representation, and then estimates a temporal attention based on resulting fine features. The temporal attention indicates the importance of each frame, which is used to re-weight the features in coarse head. At step two, a coarse GCN block updates coarse feature and estimate a spatial attention based on the resulting coarse representation, which indicates the importance of each joint. At step three, the fine grained feature is re-weighted by the spatial attention from coarse head. The intuition 



% \vspace{5cm}

%Our key idea is to sub-sample the frames at temporal dimension to maintain an additional coarse branch. Since we have reduced the frame rate, the adjacent feature frames are actually long range in their original temporal resolution. Due to sub-sampling process, we have removed the fine-grained temporal motion contexts and hence the network will focus on long range modeling. 

% To achieve this, we propose a coarse-fine dual head network. Our network consists of three modules: a backbone module extracts low level spatial and temporal features; a coarse-fine dual head module to encode both short-term and long-term dependencies; and a voting module to aggregates the short-term information and long-term information via score level fusion. We adopt the basic GCN block in previous work \cite{ms-g3d} as our backbone module. Our coarse-fine dual head module consists of a fine head and a coarse to model short-term and long-term dependencies. Specifically, in our fine head, multiple GCN blocks are concatenated to extract fine-grained motion contexts from the features with high temporal resolution. Meanwhile, in the coarse head, another bunch of GCN blocks are concatenated to extract long range motion dependencies at the down-sampled temporal resolution. To further improve the cross head context fusion and facilitate long range dependency modeling, we propose a cross head temporal attention block, which takes the feature maps from fine head to estimate a temporal attention, indicating the importance of each frame. The temporal attention is then utilized to re-weight the features in the coarse head. Moreover, we propose a cross head spatial attention mechanism, which takes the feature maps from coarse head to estimate a spatial attention, indicating the importance of each joint. The spatial attention is shared in all frames, and passes long range contexts from coarse head to fine head, to enhance fine representations. Such cross head temporal attention and spatial attention is alternately performed though forward process of dual heads, achieving efficient short-term and long-term dependency modeling. In the last stage, our voting module first predicts the action scores via each head, and then fuses the predictions via weighted sum. 





%Understanding actions from a skeleton sequence reuqires different granularities of motion patterns, existing works encodes multiple grained motion information in a unified representation, which is inefficient. Our method captures coarse grained and fine grained motion patterns in two different heads, hence is more robust to fine-grained action classes, e.g. 'reading' and 'writing'.



%\vspace{5cm}




%  Action recognition is a fundamental problem in computer vision. Recently, skeleton-based action recognition have attracted increasing attention due to the light-weight data source, high-level semantic information and robustness against complicated environment\cite{st-gcn,2s-agcn,ms-g3d}.  (Wang et al. 2018; Vemulapalli, Arrate, andChellappa 2014; Liu, Liu, and Chen 2017; Tu, Liu, and Liu2018). 
 
%  The advent of cheap motion sensors \cite{kinect,ntu_60} and effective human pose estimation algorithms  \cite{st-gcn,2s-agcn,ms-g3d} further speed up this research topic. 
%  Accurately recognizing actions from skeletal data can be very helpful in human-computer interactions, healthcare assistance and physical education\cite{xxx}. 

% related work
% Different from RGB videos, skeleton data only contains the 2D or 3D coordinates of the human key joints and lacks of image level contextual information. Hence our designed model should focus on the structure of human and motion patterns of skeletal joints. This causes the task of skeleton-based action recognition very challenging. 
% Existing works mainly focus on extracting discriminative spatial and temporal features of skeletal joints \cite{ms-aagcn,st-gcn}. Recent deep network based methods can be categorized into three types: RNNs, CNNs and GCNs. First of all, a typical method of skeleton based action recognition is RNNs\cite{xx}. Those methods first extract frame level skeletal features with a feature extractor and then modeling sequential dependencies with RNN models\cite{xx}. Typical drawback of those methods is that they compress the joint data to person-level feature in each frame and hence the intra-joint dependencies in temporal domain are hard to capture \cite{st-gcn}. The second pipeline for skeleton-based action recognition can be summarized as CNNs\cite{xxx}, which treat the joint positional data as pixels. They first flatten skeletal data of each frame to a column of pixels and then stack multiple frame data to generate an pesudo-image. Finally image-based classification CNNs are used for action recognition. However, as human skeletons lie in a non-Euclidean space, directly stacking different joints together and utilizing convolution operations may not be effective in modeling joint-level dependencies. The third framework of our task is GCNs\cite{st-gcn}, which are widely adopted in recent years due to their efficacy in spatial and temporal modeling. A milestone of GCN-based method is ST-GCN\cite{st-gcn}, which defines a sparse connected spatial-temporal graph that both considers human natural structure and temporal motion dependencies in space-time domain. Since then, many works attempted to improve the graph topology by making the graph connections learnable\cite{2s-agcn, dynamic_gcn}, adding residual layers\cite{ResGCN},  exploring contextual information between joints\cite{zhang2020context}, or introducing multi-scale spatial connections\cite{ms-g3d}.  


%allowing action recognition models to focus on understanding the action itself.
% For example, we can not infer which sport of a sport player is playing by his clothes or environments but only the skeletal sequence. This causes the task of skeleton-based action recognition very challenging. 

% In recent years, deep learning based methods have been the dominant stream for skeleton-based action recognition\cite{st-gcn, ms-aagcn,ms-g3d,decouple_gcn_cheng2020eccv,shift-gcn,ResGCN,dynamic_gcn}, where the raw skeleton sequences are first transformed into either grid-structured or graph-structured formats (e.g.,pseudo-images and graph) and then to be fed into different models (e.g., CNNs and GCNs).


%TBC


% A milestone of GCN-based method is ST-GCN\cite{st-gcn}, which first constructs a sparse connected \textbf{undirected} spatial-temporal skeleton graph and then model the spatial and temporal dependencies in a factorised/alternative way. Since then, many variants of ST-GCN are proposed.  Some works focus on improving the spatial-temporal graph topology, for example, \cite{2s-agcn,ms-aagcn,dynamic_gcn} make the spatial graph connections learnable, \cite{dgcn} constructs a directed graph, \cite{ms-g3d} constructs a multi-scale spatial-graph and together with unified pathways for robust spatial-temporal information aggregation. 
% Other works such as \cite{shift-gcn} introduce the shift convolution in graph-structured data and \cite{ResGCN} introduce a novel residual bottleneck structures to make the model more efficient. And also, \cite{zhang2020context} explores contextual information between joints\cite{zhang2020context}. \cite{mst-gcn} efficiently expands the receptive filed to long-range in spatial-temporal domain.

% \textbf{However, most of the recent works focus on spatial modeling to generate better semantic representation of human skeleton, but paid less attention on temporal modeling of dynamic frames, which is crucial to action recognition. Specifically, 
% recent SOTA methods \cite{ms-g3d,ms-aagcn,MST-GCN} capture temporal context by utilizing multiple temporal (dilated) convolutions in its 2D or 3D blocks.}



% % The key to recognize actions from skeleton sequences is to encode robust short-range and long-range temporal dependencies
%  {\color{blue}{
% %  \textbf{Motivation}
 
% A key point in skeleton-based recognition is to robustly encode spatial correlations together with  temporal motion context in the feature representations. 
% Some fine-grained actions, such as  "writing" and "typing", need model to pay more attention on fine-grained temporal dynamics while some coarse-grained actions (e.g., fall, sit down) don't need such detailed information for recognition. 
% However, most of the existing works focus on using a single model to capture holistic motion patterns for various actions. It is relatively inefficient to capture temporal coarse-level and fine-level patterns simultaneously with a bundled kernels and in some cases, such architecture suffers from recognizing fine-grained actions such as "writing" and "typing".
% As shown in Figure xxx \ref{Fig.Ads}, to remedy/alleviate the above drawbacks, we propose a dual head architecture which can effectively learn a  robust representations of the input skeleton sequences from coarse-level and fine-level.  


% Our network consists of three modules: a backbone module extracts low level spatial and temporal features; a coarse-and-fine dual head module to encode motion patterns from two temporal perspectives;  a cross-head communication module used for two heads to help each other and enhance the representations of two heads mutually; a late-fusion module for coarse-fine combination
% Specifically,  we adopt the basic Spatial-Temporal Graph Convolution block (STGC-block) in previous work \cite{ms-g3d} as our backbone module. Such basic blocks are also used in other part.
% In our fine head, multiple STGC-blocks are concatenated to extract fine-grained motion contexts from the features with high temporal resolution. Meanwhile, in the coarse head, another bunch of STGC-blocks are concatenated to extract coarse-grained motion dependencies at the down-sampled temporal resolution. 
% To further improve the cross head context fusion and facilitate the representation modeling, we propose a cross-head communication module which contains a temporal attention block and a spatial attention block. Temporal attention block takes the feature maps from fine head to estimate a temporal attention, indicating the importance of each frame which is then utilized to re-weight the features in the coarse head in temporal dimension. Spatial attention block takes the feature maps from coarse head to estimate a spatial attention, indicating the importance of each joint.  The spatial attention is shared in all frames, and passes relative robust spatial contexts from coarse head to fine head. Such cross head temporal attention and spatial attention is alternately performed through forward process of dual heads, achieving efficient spatial and temporal dependency modeling. 
% In the end, each head predicts a probability of each action class, and we fuse the estimated scores to generate final predictions. 


% Specifically,  we adopt the basic Spatial-Temporal Graph Convolution block (STGC-block) in previous work \cite{ms-g3d} as our backbone module. A fine head extracts features at a high temporal resolution, and a coarse head extracts features at low temporal resolution. 
%  During forward process, the fine head focuses on extracting fine-grained temporal contexts, and simultaneously, the coarse head focuses on capturing coarse-grained temporal dependencies. An alternative cross-head communication mechanism is designed for mutually enhancing feature representations by leveraging their individual advantages. (Finer Temporal Attention of fine head  and stronger Spatial Attention of Coarse head). 


% To achieve this, we propose a coarse-fine dual head network. Our network consists of three modules: a backbone module extracts low level spatial and temporal features; a coarse-fine dual head module to encode both short-term and long-term dependencies; and a voting module to aggregates the short-term information and long-term information via score level fusion. We adopt the basic GCN block in previous work \cite{ms-g3d} as our backbone module. Our coarse-fine dual head module consists of a fine head and a coarse to model short-term and long-term dependencies. Specifically, in our fine head, multiple GCN blocks are concatenated to extract fine-grained motion contexts from the features with high temporal resolution. Meanwhile, in the coarse head, another bunch of GCN blocks are concatenated to extract long range motion dependencies at the down-sampled temporal resolution. To further improve the cross head context fusion and facilitate long range dependency modeling, we propose a cross head temporal attention block, which takes the feature maps from fine head to estimate a temporal attention, indicating the importance of each frame. The temporal attention is then utilized to re-weight the features in the coarse head. Moreover, we propose a cross head spatial attention mechanism, which takes the feature maps from coarse head to estimate a spatial attention, indicating the importance of each joint. The spatial attention is shared in all frames, and passes long range contexts from coarse head to fine head, to enhance fine representations. Such cross head temporal attention and spatial attention is alternately performed though forward process of dual heads, achieving efficient short-term and long-term dependency modeling. In the last stage, our voting module first predicts the action scores via each head, and then fuses the predictions via weighted sum. 

% We adopt the basic Spatial-Temporal Graph Convolution block (STGC-block) in previous work \cite{ms-g3d} as our backbone module. 
% To further improve the cross head context fusion and facilitate long range dependency modeling, we propose a cross head temporal attention block, which takes the feature maps from fine head to estimate a temporal attention, indicating the importance of each frame. The temporal attention is then utilized to re-weight the features in the coarse head. Moreover, we propose a cross head spatial attention mechanism, which takes the feature maps from coarse head to estimate a spatial attention, indicating the importance of each joint. The spatial attention is shared in all frames, and passes long range contexts from coarse head to fine head, to enhance fine representations.

% }}



% \vspace{5cm}
% The key to recognize actions from skeleton sequences is to encode short-term and long-term temporal motion context in the feature representations. On the one hand, many actions are discriminative by subtle temporal movements of pivotal key points; on the other hand, long range dependency in temporal dimension is crucial for action recognition. Existing works address the problem by concatenating multiple dilated temporal convolutions and 3D graph blocks with multiple window sizes\cite{ms-g3d,MST-GCN}. Despite the promising performance they achieve, there still exist several drawbacks in the design of their architectures. Specifically, in MS-G3D, the factorized pathway and G3D blocks have different temporal kernel sizes/receptive fields, hence that each graph node receives more messages from nearby nodes than long distant nodes. As a result, the aggregating process is biased to short-range dependency. Similarly in MST-GCN, long range contexts is estimated based on short range contexts. In addition, the short range and long range temporal context are mixed in their representation, hence the features will encode more local information than long range contexts due to biased aggregation.

% \textbf{To sufficiently capture long range dependencies,} we propose a dual head framework to remedy the above drawbacks. Our key idea is to sub-sample the frames at temporal dimension to maintain an additional coarse branch. Since we have reduced the frame rate, the adjacent feature frames are actually long range in their original temporal resolution. Due to sub-sampling process, we have removed the fine-grained temporal motion contexts and hence the network will focus on long range modeling. 

% Specifically, our framework has two heads: a fine head extracts features at a high temporal resolution, and a coarse head extracts features at low temporal resolution. During forward process, the fine head focuses on extracting fine-grained temporal contexts, and parallel the coarse head focuses on long range temporal dependencies. In the end, each head predicts a probability of each action class, and we fuse the estimated scores to generate final predictions. 

% To achieve this, we propose a coarse-fine dual head network. Our network consists of three modules: a backbone module extracts low level spatial and temporal features; a coarse-fine dual head module to encode both short-term and long-term dependencies; and a voting module to aggregates the short-term information and long-term information via score level fusion. We adopt the basic GCN block in previous work \cite{ms-g3d} as our backbone module. Our coarse-fine dual head module consists of a fine head and a coarse to model short-term and long-term dependencies. Specifically, in our fine head, multiple GCN blocks are concatenated to extract fine-grained motion contexts from the features with high temporal resolution. Meanwhile, in the coarse head, another bunch of GCN blocks are concatenated to extract long range motion dependencies at the down-sampled temporal resolution. To further improve the cross head context fusion and facilitate long range dependency modeling, we propose a cross head temporal attention block, which takes the feature maps from fine head to estimate a temporal attention, indicating the importance of each frame. The temporal attention is then utilized to re-weight the features in the coarse head. Moreover, we propose a cross head spatial attention mechanism, which takes the feature maps from coarse head to estimate a spatial attention, indicating the importance of each joint. The spatial attention is shared in all frames, and passes long range contexts from coarse head to fine head, to enhance fine representations. Such cross head temporal attention and spatial attention is alternately performed though forward process of dual heads, achieving efficient short-term and long-term dependency modeling. In the last stage, our voting module first predicts the action scores via each head, and then fuses the predictions via weighted sum. 




%现在的方法，MS-G3D，同时考虑了short range和long range的dependency，在每一个block里，利用了mutliple dilated convolutions with different dilation rates, and multiple G3D components with different window sizes to capture both short range and long range dependency. However, is this blocks, long range dependency is not sufficiently modeled like short-range, since that times of short range message passing is much more than long range message passing. It makes the network 
% In this work, we propose a novel approach to skeleton-based action recognition in order to perform spatial and temporal modeling in an effective way. Our key idea is to utilize two branches of networks, one branch focuses on extracting joint-level semantic features, and the other branch focuses on extracting detailed temporal motion information. In the end, we are able to fuse the outputs of both networks, performing joint spatial and temporal inference. 

% {
% \color{blue} Motivation 

% %粗细粒度的结合在Action Recognition中的作用
% % 1. 粗粒度的网络如何从粗粒度的动作中提取 coarse-grained feature
% % 2. 细粒度网络如何识从细粒度的动作中提取 fine-grained feature
% % 3. 为什么要两者结合
% Modelling robust temporal dependencies from various skeleton sequences is a fundamental challenge in skeleton-based action recognition. Most existing methods often overlook the hierarchical granularities of actions in time domain and thus fail to extract discriminative representations for fine-grained actions (eg. reading, writing and eating food). 
% (or modelling discriminative dependencies for different action granularities in temporal dimension)
% In this paper, we propose a novel attention-enhanced cross-fine dual head networks (C2F-DH Net)for robust temporal modelling by exploring different action granularities. 

% Our C2F-DH Net consists of three main stages:

% 1) We first construct A coarse representation net (CRN) to model long-range temporal dependencies, A Fine context proposal net (FCPN) which can  produce finer context information. 

% 2) Then we apply a cross-branch attention mechanism between the two branches. The fine head can refine coarse head by producing finer temporal context, while the coarse head can in turn provide fine head with coarse spatial configuration information. Finally, these two branches can refine each other along with the model optimization process. 

% 3) Finally, a  voting mechanism is adopted aims at taking the most advantages of these two different granularities of representations. This voting mechanism is accompanied with two losses, thus our model can learn the fine-grained features and coarse-grained features individually along with the optimization process of the model. The final voting results of two heads is thus robust both for  fine-level and coarse-level inputs.

% % }
% \vspace{4cm}
% To achieve this, we first utilize a GCN block \cite{ms-g3d} to generate features of input skeleton sequence, and then propose a dual head network based on the backbone feature extractor, where each head is associated with spatial or temporal modeling. The spatial head aims at extracting semantic features between different joints while ignoring fine-grained temporal context, and the temporal head explores finer temporal motions while weakening spatial dependencies. To this end, we adopt two slightly different modification from the basic GCN block \cite{ms-g3d}. In the spatial head, we down sample the feature maps in temporal dimension, the latter computations are based on the resulting features. In addition, we reduce the kernel sizes and dilation rates of the temporal convolutions. In this way the feature maps carry coarse temporal motion context, and hence our network can focus more on spatial modeling. As for the temporal head, we borrow the idea of the SlowFast Network\cite{slowfast}, which decreases the dimensions of feature channels. In skeletal data, each joint has its semantic meaning, hence the joint positional data are naturally aligned in different temporal frames. Extracting temporal movements of the same joint or nearby joints in different frames is much easier than extracting abstract spatial features, hence reducing feature channels can enforce the network encode less spatial context but focus on temporal motions. To sufficient exploit our spatial head and temporal head, we further propose a novel attention mechanism to enhance the spatial and temporal features. Finally, each head generates a probabilistic prediction of action classes. The final prediction is generated by combing the voting of both heads.

% Specifically, the spatial head consists of a sub-sampling layer followed by two modified GCN blocks and a prediction layer. The subsampling layer is used to downsample feature maps at temporal resolution. For the GCN structure, we decrease the number of G3D pathways in MS-G3D, aiming to weaken the 3D or temporal modeling. We also decrease the dilation rates and kernel sizes of the temporal convolution blocks or G3D blocks. The temporal head consists of an embedding layer to decrease feature channels and two MS-G3D blocks, and a prediction layers. To further enhance the learned temporal and spatial context, we propose a cross head attention mechanism, which utilizes the spatial head to estimates an spatial joint-level attention for each joint and the temporal head to estimate the temporal attention of each temporal frame. The estimated attentions are used to enhance spatial or temporal features of the other bead in a residual way. Finally, the predictions of both heads are used to voting for final prediction.

% \textcolor{blue}{I'm not sure whether should remain this or move it to section 2:} Our method is different from the SlowFast Network\cite{slowfast}. First of all, we generate the slow branch by subsampling the feature maps instead of raw data frames. Such structure is more like the Temporal Pyramid Network\cite{tpn} or HRNet\cite{hrnet}. In addition, our final prediction is generated by voting of both heads, instead of the fusion of each head's feature maps. We will describe the related work in detail in the next section. \textcolor{red}{By modifying the G3D blocks, our network has fewer parameters than MS-G3D.}.




\begin{figure*}[t]
	\centering
	\includegraphics[width=1.\textwidth]{paperSec/imgs/Overview_Framework/Overview_Framework_finalize.pdf}
	\caption{Overview of our proposed framework. We first utilize a STGC block to generate backbone features of skeleton data, and then use a coarse head to capture coarse grained motion patterns, a fine head to encode fine-grained subtle temporal movements. Cross head spatial and temporal attentions are exploited to mutually enhance  feature representations. Finally each head generates a probabilistic prediction of actions and the ultimate estimation is given by fusion of both predictions.}
	\label{fig:Overall_Framework}
\end{figure*}

% \begin{figure*}[t]
% 	\centering
% 	\includegraphics[width=1.\textwidth]{paperSec/imgs/Overview_Framework/Overview_Framework_Refined_2.pdf}
% 	\caption{Overview of our proposed framework. We first utilize a STGC block to generate backbone features of skeleton data, and then use a coarse head to capture coarse grained motion patterns, a fine head to encode fine-grained subtle temporal movements. Cross head spatial and temporal attentions are exploited to mutually enhance  feature representations. Finally each head generates a probabilistic prediction of actions and the ultimate estimation is given by fusion of both predictions.}
% 	\label{fig:Overall_Framework}
% \end{figure*}



==> paperSec/relatedwork.tex <==
\begin{figure*}[!t]
	\centering
	\includegraphics[width=0.95\textwidth]{paperSec/imgs/Overview_Framework/Overview_Framework_finalize.pdf}
	\vspace{-0.3cm}
	\caption{\small Overview of our proposed framework. We first utilise a STGC block to generate backbone features of skeleton data, and then use a coarse head to capture coarse-grained motion patterns, a fine head to encode fine-grained subtle temporal movements. Cross head spatial and temporal attentions are exploited to mutually enhance  feature representations. Finally each head generates a probabilistic prediction of actions and the ultimate estimation is given by fusion of both predictions.}
	\vspace{-0.2cm}
	\label{fig:overview}
	\Description{}
\end{figure*}


% \begin{figure*}[t]
% 	\centering
% 	\includegraphics[width=1.\textwidth]{paperSec/imgs/Overview_Framework_Version3.pdf}
% 	\caption{Overview of our proposed framework. We first utilise a MS-G3D block to generate backbone features of skeleton data, and then use a spatial head to focus on spatial modeling, a temporal head to focus on temporal modeling. Cross head spatial and temporal attentions are exploited to enhance spatial and temporal features. Finally each head generates a probabilistic prediction of actions and the ultimate estimation is given by voting of both predictions.}
% 	\label{fig:Overall_Framework}
% \end{figure*}


% \begin{figure*}[t]
% 	\centering
% 	\includegraphics[width=1.\textwidth]{paperSec/imgs/Overview_Framework_Version_2.pdf}
% 	\caption{Overview of our proposed framework. We first utilise a MS-G3D block to generate backbone features of skeleton data, and then use a spatial head to focus on spatial modeling, a temporal head to focus on temporal modeling. Cross head spatial and temporal attentions are exploited to enhance spatial and temporal features. Finally each head generates a probabilistic prediction of actions and the ultimate estimation is given by voting of both predictions.}
% 	\label{fig:Overall_Framework_v2}
% \end{figure*}



\section{Related Work}
%  1. the difference between video-based action recognition and skeleton-based action recognition
 
%  2. GCN-based methods brief intro
\subsection{Skeleton-based Action Recognition}

% Existing works mainly focus on extracting discriminative spatial and temporal features of skeletal joints \cite{ms-aagcn,st-gcn}. Recent deep network based methods can be categorized into three types: RNNs, CNNs and GCNs. First of all, a typical method of skeleton based action recognition is RNNs\cite{xx}. Those methods first extract frame level skeletal features with a feature extractor and then modeling sequential dependencies with RNN models\cite{xx}. Typical drawback of those methods is that they compress the joint data to person-level feature in each frame and hence the intra-joint dependencies in temporal domain are hard to capture \cite{st-gcn}. The second pipeline for skeleton-based action recognition can be summarized as CNNs\cite{xxx}, which treat the joint positional data as pixels. They first flatten skeletal data of each frame to a column of pixels and then stack multiple frame data to generate an pesudo-image. Finally image-based classification CNNs are used for action recognition. However, as human skeletons lie in a non-Euclidean space, directly stacking different joints together and utilizing convolution operations may not be effective in modeling joint-level dependencies. The third framework of our task is GCNs\cite{st-gcn}, which are widely adopted in recent years due to their efficacy in spatial and temporal modeling. A milestone of GCN-based method is ST-GCN\cite{st-gcn}, which defines a sparse connected spatial-temporal graph that both considers human natural structure and temporal motion dependencies in space-time domain. Since then, many works attempted to improve the graph topology by making the graph connections learnable\cite{2s-agcn, dynamic_gcn}, adding residual layers\cite{ResGCN},  exploring contextual information between joints\cite{zhang2020context}, or introducing multi-scale spatial connections\cite{ms-g3d}. 

%Skeleton-based action recognition have attracted increasing attention due to the robustness against body scales, view-points and backgrounds. 

Conventional methods for skeleton-based action recognition usually design hand-crafted features to model the human body \cite{vemulapalli2014human,hu2015jointly,hussein2013human}. However, these methods mainly focus on exploiting the relative 3D rotations and translations between joints and suffer from complicated design process. Recent deep network based methods can be categorized into three types: RNNs, CNNs and GCNs. 
%With the development of the deep learning, data-driven methods have been proven more effective than those methods based on hand-crafted features. 
%Those methods first extract frame level skeletal features with a feature extractor and then model sequential dependencies with RNN models\cite{}


% 			The first group involves explicitly capturing the sequence properties of actions and modelling their time dependences using RNN or LSTM \cite{du2015hierarchical,ntu_60,liu2016spatio,song2017end,zheng2019relational}. Attempts based on RNN model include constructing an adaptive tree-structured RNN architecture \cite{li2017adaptive} or designing a view adaptation scheme to automatically regulate observation viewpoints during the occurrence of an action \cite{zhang2017view}. As an alternative way to capturing sequential information, LSTM networks have been employed to mine global informative joints \cite{liu2017global}; to extract co-occurrence features of skeleton sequences \cite{zhu2016co} or to learn stacked temporal dynamics \cite{si2018skeleton}. 
	

RNN-based methods first extract frame level skeletal features with a feature extractor and then model sequential dependencies with RNN models  \cite{du2015hierarchical,ntu_60,liu2016spatio, li2017adaptive, zhang2017view}. For example, \cite{li2017adaptive} constructed an adaptive tree-structured RNN architecture based on RNN model. \cite{zhang2017view} designed a view adaptation scheme to automatically regulate observation viewpoints during the occurrence of an action. LSTM networks have also been employed to mine global informative joints \cite{liu2017global}; to extract co-occurrence features of skeleton sequences \cite{zhu2016co} or to learn stacked temporal dynamics \cite{si2018skeleton}. 


% [?8]  use  a hierarchical bidirectional RNN model to identify the skeleton sequence,  which  divides  the  human  body  into  different  parts and  sends  them  to  different  sub-networks.  
% %Song  et  al. [?11] embed  a  spatiotemporal  attention  module  in  LSTM-based model,  so  that  the  network  can  automatically  pay  attention to  the  discriminant  spatio temporal  region  of  the  skeleton sequence. Zhang et al. [?12] introduce the mechanism of view transformation in an LSTM-based model, which automatically translates the skeleton data into a more advantageous angle for action recognition. Si et al. 
% %[?36] propose a model with spatial reasoning (SRN) and temporal stack learning (TSL), where the SRN can capture the structural information between different body  parts  and  the  TSL  can  model  the  detailed  temporal dynamics.[23] divides the cell of LSTM into five part-cells which correspond to five body parts respectively. 
% [34] proposed a view adaptation scheme to automatically regulate observation viewpoints during the occurrence of an action. 
% %Typical drawback of those methods is that they compress the joint data to person-level feature in each frame and hence the intra-joint dependencies in temporal domain are hard to capture \cite{st-gcn}.

% 			The second group exploits various predefined transformation rules to treat the input skeleton as a pseudo-image, which is then extracted and purified by a CNN \cite{ke2017new,kim2017interpretable}. Standard works include skepxels \cite{liu2019skepxels}, joint-wise co-occurence feature learning \cite{li2018co}, and enhanced skeleton visualization model \cite{liu2017enhanced}. However, conventional CNNs are usually insufficient to accurately express the vertex information located in non-Euclidean space. 


CNN-based methods usually formulate the skeleton sequences as a pseudo-image, where the coordinate of each skeleton joint (x,y,z) is regarded as three channels of the image. Then a CNN is designed to directly classify the transformed image into action categories. \cite{li2018co} proposes a co-occurrence feature learning framework. \cite{kim2017interpretable} use  a  one-dimensional  residual CNN  to  identify  skeleton  sequences  where  the  coordinates of  joints  are  directly  concatenated. \cite{liu2017enhanced} propose 10 kinds of spatiotemporal images for skeleton encoding, and enhance  these  images  using  visual  and  motion  enhancement methods. 
%The success of CNNs is attributed to their strong capability in feature representation. 

%the  CNN-based  methods are  generally  more  popular  than  the  RNN-based  methods because the CNNs have better parallelizability and are easier for  training.  

% However, both the RNNs and CNNs lost the skeleton topology information because the skeleton data are naturally structed in the form of graphs rather than a vector sequence or a 2D grid. Recently, GCN-based methods are proposed to deal with irregularly structured graphs like skeleton data. Given skeleton data with N joints, the graph topology can be well represented by an NxN adjacency matrix A. The key of GCN-based methods lied in the design of graph topology Yan et al \cite{st-gcn} propose a milestone work which introduce GCN into Skeleton-based Action recognition. \cite{2s-agcn} propose a adaptive attention module to learn non-local dependecies in spatial dimension. Following works pay much attention on designing spatial topology  and neglect the temporal information modelling. Then, \cite{ms-g3d} propose a multi-scale aggregation methods which can effectively aggregate spatial information and use multiple temporal windows to capture temporal dimensions. 
However, both the RNNs and CNNs lost the skeleton topology information because the skeleton data are naturally strucutilisetured in the form of graphs rather than a vector sequence or a 2D grid. Recent works utilise GCNs\cite{st-gcn,2s-agcn} for spatial and temporal modeling. A milestone of GCN-based method is ST-GCN\cite{st-gcn}, which defines a sparse connected spatial-temporal graph that both considers human natural structure and temporal motion dependencies in space-time domain. Since then, many works follow GCNs for skeleton-based action recognition. 2s-AGCN\cite{2s-agcn} proposes an adaptive attention module to learn non-local dependencies in spatial dimension. \cite{zhang2020context} explores contextual information between joints. \cite{ms-aagcn} further introduces spatial and temporal attentions in the GCN. \cite{shift-gcn} introduces the shift convolution in graph-structured data. \cite{ms-g3d} proposes a multi-scale aggregation methods which can effectively aggregate spatial information and use multiple temporal windows to capture temporal dimensions. \cite{dynamic_gcn} proposes a context-enriched module for better graph connection. \cite{ResGCN} proposes to utilise multiple data modality in a single model. \cite{MST-GCN-AAAI2021} proposes multi-scale spatial temporal graph for long range modeling. However, existing GCN based methods represent different granularities of motion information in a unified representation. Our method utilises two heads to focus on coarse grained and fine grained motion patterns separately and hence is more effective.
%\vspace{-0.3cm}

%Following works pay much attention on designing spatial topology  and neglect the temporal information modelling. Then, \cite{ms-g3d} propose a multi-scale aggregation methods which can effectively aggregate spatial information and use multiple temporal windows to capture temporal dimensions.
%Since then, many works attempted to improve the graph topology by making the graph connections learnable\cite{2s-agcn,ms-aagcn,dynamic_gcn}, adding residual layers\cite{ResGCN},  exploring contextual information between joints\cite{zhang2020context}, or introducing multi-scale spatial connections\cite{ms-g3d}. 
%However, the  stack of temporal convolutional operations can not effectively capture the visual tempos . The visual tempo of action should be considered for fine-grained action classification.
%Visual tempo characterizes the dynamics and the temporal scale of an action, which actually describes how fast an action goes. Modeling such visual tempos of different actions facilitates their recognition.
% A milestone of GCN-based method is ST-GCN\cite{st-gcn}, which first constructs a sparse connected \textbf{undirected} spatial-temporal skeleton graph and then model the spatial and temporal dependencies in a factorised/alternative way. Since then, many variants of ST-GCN are proposed.  Some works focus on improving the spatial-temporal graph topology, for example, \cite{2s-agcn,ms-aagcn,dynamic_gcn} make the spatial graph connections learnable, \cite{dgcn} constructs a directed graph, \cite{ms-g3d} constructs a multi-scale spatial-graph and together with unified pathways for robust spatial-temporal information aggregation. 
% Other works such as \cite{shift-gcn} introduce the shift convolution in graph-structured data and \cite{ResGCN} introduce a novel residual bottleneck structures to make the model more efficient. And also, \cite{zhang2020context} explores contextual information between joints\cite{zhang2020context}. \cite{mst-gcn} efficiently expands the receptive filed to long-range in spatial-temporal domain.
%In our work, we proposed a novel dual head network which can effectively capture spatial information as well as modelling  visual tempos of different actions and temporal information individually. Slow branch capture the

\subsection{Video-based Action Recognition}
Some video-based action recognition methods focus on temporal modeling at different pathways or temporal resolutions. SlowFast Networks\cite{feichtenhofer2019slowfast} "factorize" spatial and temporal inference in two different pathways. Temporal Pyramid Network\cite{yang2020temporal} explores different visual tempos by fusing features at different stages with different temporal resolutions. Recent Coarse-Fine networks\cite{kahatapitiya2021coarse} propose a re-sampling module to improve long range dependencies. However, different motion granularities are not sufficiently explored in skeleton-based action recognition. Due to the lack of image level context, we need to carefully design the networks for each granularity. In addition, we propose a cross-head attention strategy to communicate each head with another, resulting in an effective dual granularity reasoning.


%Video-based action recognition focus on the temporal modelling to capture the motion information 
%Optical Flow
%SlowFast 
%TSM 
%TPN

%Temporal Modelling Methods

%RNNs CNNs GCNs(Focus on GCNs )


% \subsection{Graph Convolutional  Networks}

% Skeleton-based action recognition has been dominated by deep learning-based methods. They have been proven more effective than those methods based on hand-crafted features [29,30,32]. Inspired by the booming graph-based methods, Yan, et al.[31]firstly introduce GCN into the skeleton-based action recognition task, and propose the ST-GCN to model the spatial configurations and temporal dynamics of skeletons synchronously. Following this work, Song et al.[27] aims to solve the occlusion problem in this task, and propose a multi-stream GCN to extract rich features from more activated skeleton joints. Shi et al.[23] utilise a Non-local method into a two-stream GCN model, which significantly improves the model’s accuracy. In MS-GCN, 
% Reference Shift-GCN, MS-AAGCN, MS-G3D,  Dynamic-GCN, PA-Res-GCN, and finally MST-GCN, 

% However, these well-performance models are usually based on multi-stream structures, which need to tune a larger amount of parameters with higher computational costs.Therefore, how to reduce the complexity of the GCN model is still a challenging problem for 3D skeleton based action recognition.



% Skeleton-based action recognition has been dominated by deep learning-based methods. They have been proven more effective than those methods based on hand-crafted features [29,30,32]. Due to its compactness to the RGB-based representations, action recognition based on skeleton data has received increasing attentions. In an earlier work [13], a convolutional co-occurrence feature learning framework is proposed, where a hierarchical methodology is employed to gradually aggregate different levels of contextual information. The study in[34] designs a view adaptive model to automatically regulate observation viewpoints during the occurrence of an action, so as to obtain the view invariant representations of human actions. Inspired by the booming graph-based methods, Yan, et al.[31]firstly introduce GCN into the skeleton-based action recognition task, and propose the ST-GCN to model the spatial configurations and temporal dynamics of skeletons synchronously. Following this work, Song et al.[27] aims to solve the occlusion problem in this task, and propose a multi-stream GCN to extract rich features from more activated skeleton joints. Shi et al.[23] utilise a Non-local method into a two-stream GCN model, which significantly improves the model’s accuracy. In MS-GCN, 
% Reference Shift-GCN, MS-AAGCN, MS-G3D,  Dynamic-GCN, PA-Res-GCN, and finally MST-GCN, 

% However, these well-performance models are usually based on multi-stream structures, which need to tune a larger amount of parameters with higher computational costs.Therefore, how to reduce the complexity of the GCN model is still a challenging problem for 3D skeleton based action recognition.

